GreenLLM: Disaggregating Large Language Model Serving on Heterogeneous GPUs for Lower Carbon Emissions

LLMs have been widely adopted across many real-world applications. However, their widespread use comes with significant environmental costs due to their high computational intensity and resource demands. Specifically, this has driven the development of new generations of high-performing GPUs, exacerbating the problem of electronic waste and accelerating the premature disposal of devices. To address this problem, this paper focuses on reducing the carbon emissions of LLM serving by reusing older, low-performing GPUs. We present GreenLLM, an SLO-aware LLM serving framework designed to minimize carbon emissions by reusing older GPUs. GreenLLM builds on two identified use cases that disaggregate specific computations onto older GPUs, reducing carbon emissions while meeting performance goals. To deepen our understanding of the potential carbon savings from disaggregation, we also provide a theoretical analysis of its relationship with carbon intensity and GPU lifetime. Our evaluations show that GreenLLM reduces carbon emissions by up to 40.6% compared to running standard LLM serving on new GPU only, meeting latency SLOs for over 90% of requests across various applications, latency requirements, carbon intensities, and GPU lifetimes.

==> fig/tikz/dsd_carbon_per_token/dsd_carbon_per_token_humaneval_1b.tex <==
\begin{tikzpicture}[
every axis/.style={
    style={font=\footnotesize},
    ybar stacked,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
    },
    scaled y ticks=false,
    % ymode=log,
    ylabel shift={-3pt},
    bar width=4pt,
    clip=false,
    height=4.5cm,
    width=1\hsize,
    ymin=0,
    ymax=0.00006,
    ytick={0.00002, 0.00004, 0.00006},
    yticklabels = {2e-5, 4e-5, 6e-5},
    % ytick = {},
    % xtick=data,
    % x tick label style={align=center, text width=.8cm}, 
    xtick={0,...,10},
    xticklabels = {1, 2, 4,6, 8, 10, 14,18},
    xlabel={QPS},
    % xmode=log,
    y label style={align=center, text width=3cm}, % Setting alignment is needed to add a line break in axis label
    ylabel={Carbon Emission\\(gCO\textsubscript{2}/token)},
    % tickwidth= 5pt,
    xtick style={draw=none},
    ymajorgrids=true,
    % grid style=dashed,
    legend columns=1,
    legend cell align=left,
    legend style={
        cells={align=left},
        anchor=north,
        at={(0.8,0.97)},
        draw=none,
        fill=none,
        column sep=1ex,
    },
    legend image code/.code={%
        \draw[#1,draw=none] (0cm,-0.07cm) rectangle (0.17cm,0.12cm);
    }
}
]

\begin{axis}[bar shift=6pt]
\addplot+[draw=none,fill=kaito,opacity=0.25] table[col sep=comma, y=v100_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_1b.csv};
\addplot+[draw=none,fill=orange] table[col sep=comma, y=v100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_1b.csv};\label{dsd_he_1b_v100}

\end{axis}



\begin{axis}[hide axis, bar shift=0pt]
\addplot+[
    draw=none,
    fill=kaito,opacity=0.25] table[col sep=comma, y=t4_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_1b.csv};\label{dsd_he_1b_a100_dist};
\addplot+[draw=none,fill=green!70!black] table[col sep=comma, y=t4_carbon_pertoken,   x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_1b.csv};\label{dsd_he_1b_plot_t4}

\end{axis}


\begin{axis}[hide axis, bar shift=-6pt]

\addplot+[draw=none,fill=blue] table[col sep=comma, y=a100_std,  x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_1b.csv};

\addlegendentry{A100 only}
\addlegendimage{/pgfplots/refstyle=dsd_he_1b_plot_t4}\addlegendentry{T4}
\addlegendimage{/pgfplots/refstyle=dsd_he_1b_v100}\addlegendentry{V100}
\addlegendimage{/pgfplots/refstyle=dsd_he_1b_a100_dist}\addlegendentry{A100 Dist}


\end{axis}



\end{tikzpicture}

==> fig/tikz/dsd_carbon_per_token/dsd_carbon_per_token_humaneval_300m.tex <==
\begin{tikzpicture}[
every axis/.style={
    style={font=\footnotesize},
    ybar stacked,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
    },
    scaled y ticks=false,
    % ymode=log,
    ylabel shift={-3pt},
    bar width=4pt,
    clip=false,
    height=4.5cm,
    width=1\hsize,
    ymin=0,
    ymax=0.00006,
    ytick={0.00002, 0.00004, 0.00006},
    yticklabels = {2e-5, 4e-5, 6e-5},
    % ytick = {},
    % xtick=data,
    % x tick label style={align=center, text width=.8cm}, 
    xtick={0,...,10},
    xticklabels = {1, 2, 4,6, 8, 10, 14,18},
    xlabel={QPS},
    % xmode=log,
    y label style={align=center, text width=3cm}, % Setting alignment is needed to add a line break in axis label
    ylabel={Carbon Emission\\(gCO\textsubscript{2}/token)},
    % tickwidth= 5pt,
    xtick style={draw=none},
    ymajorgrids=true,
    % grid style=dashed,
    legend columns=1,
    legend cell align=left,
    legend style={
        cells={align=left},
        anchor=north,
        at={(0.8,0.97)},
        draw=none,
        fill=none,
        column sep=1ex,
    },
    legend image code/.code={%
        \draw[#1,draw=none] (0cm,-0.07cm) rectangle (0.17cm,0.12cm);
    }
}
]

\begin{axis}[bar shift=6pt]
\addplot+[draw=none,fill=kaito,opacity=0.25] table[col sep=comma, y=v100_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_300m.csv};
\addplot+[draw=none,fill=orange] table[col sep=comma, y=v100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_300m.csv};\label{dsd_he_300m_v100}

\end{axis}



\begin{axis}[hide axis, bar shift=0pt]
\addplot+[
    draw=none,
    fill=kaito,opacity=0.25] table[col sep=comma, y=t4_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_300m.csv};\label{dsd_he_300m_a100_dist};
\addplot+[draw=none,fill=green!70!black] table[col sep=comma, y=t4_carbon_pertoken,   x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_300m.csv};\label{dsd_he_300m_plot_t4}

\end{axis}


\begin{axis}[hide axis, bar shift=-6pt]

\addplot+[draw=none,fill=blue] table[col sep=comma, y=a100_std,  x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/humaneval_carbon_per_token_300m.csv};

\addlegendentry{A100 only}
\addlegendimage{/pgfplots/refstyle=dsd_he_300m_plot_t4}\addlegendentry{T4}
\addlegendimage{/pgfplots/refstyle=dsd_he_300m_v100}\addlegendentry{V100}
\addlegendimage{/pgfplots/refstyle=dsd_he_300m_a100_dist}\addlegendentry{A100 Dist}


\end{axis}



\end{tikzpicture}

==> fig/tikz/dsd_carbon_per_token/dsd_carbon_per_token_longbench_1b.tex <==
\begin{tikzpicture}[
every axis/.style={
    style={font=\footnotesize},
    ybar stacked,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
    },
    scaled y ticks=false,
    % ymode=log,
    ylabel shift={-3pt},
    bar width=4pt,
    clip=false,
    height=4.5cm,
    width=1\hsize,
    ymin=0,
    ymax=0.000022,
    ytick={0.00001, 0.00002},
    yticklabels = {1e-5, 2e-5},
    % ytick = {},
    % xtick=data,
    % x tick label style={align=center, text width=.8cm}, 
    xtick={0,...,7},
    xticklabels = {0.5, 0.75, 1, 1.25, 1.5, 2,  2.5, 2.75},
    xlabel={QPS},
    % xmode=log,
    y label style={align=center, text width=3cm}, % Setting alignment is needed to add a line break in axis label
    ylabel={Carbon Emission\\(gCO\textsubscript{2}/token)},
    % tickwidth= 5pt,
    xtick style={draw=none},
    ymajorgrids=true,
    % grid style=dashed,
    legend columns=1,
    legend cell align=left,
    legend style={
        cells={align=left},
        anchor=north,
        at={(0.8,0.97)},
        draw=none,
        fill=none,
        column sep=1ex,
    },
    legend image code/.code={%
        \draw[#1,draw=none] (0cm,-0.07cm) rectangle (0.17cm,0.12cm);
    }
}
]

\begin{axis}[bar shift=6pt]
\addplot+[draw=none,fill=kaito,opacity=0.25] table[col sep=comma, y=v100_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_1b.csv};
\addplot+[draw=none,fill=orange] table[col sep=comma, y=v100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_1b.csv};\label{dsd_1b_1b_v100}

\end{axis}



\begin{axis}[hide axis, bar shift=0pt]
\addplot+[
    draw=none,
    fill=kaito,opacity=0.25] table[col sep=comma, y=t4_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_1b.csv};\label{dsd_1b_1b_a100_dist};
\addplot+[draw=none,fill=green!70!black] table[col sep=comma, y=t4_carbon_pertoken,   x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_1b.csv};\label{dsd_1b_1b_plot_t4}

\end{axis}


\begin{axis}[hide axis, bar shift=-6pt]

\addplot+[draw=none,fill=blue] table[col sep=comma, y=a100_std,  x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_1b.csv};

\addlegendentry{A100 only}
\addlegendimage{/pgfplots/refstyle=dsd_1b_1b_plot_t4}\addlegendentry{T4}
\addlegendimage{/pgfplots/refstyle=dsd_1b_1b_v100}\addlegendentry{V100}
\addlegendimage{/pgfplots/refstyle=dsd_1b_1b_a100_dist}\addlegendentry{A100 Dist}


\end{axis}



\end{tikzpicture}

==> fig/tikz/dsd_carbon_per_token/dsd_carbon_per_token_longbench_300m.tex <==
\begin{tikzpicture}[
every axis/.style={
    style={font=\footnotesize},
    ybar stacked,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
    },
    scaled y ticks=false,
    % ymode=log,
    ylabel shift={-3pt},
    bar width=4pt,
    clip=false,
    height=4.5cm,
    width=1\hsize,
    ymin=0,
    ymax=0.000022,
    ytick={0.00001, 0.00002},
    yticklabels = {1e-5, 2e-5},
    % ytick = {},
    % xtick=data,
    % x tick label style={align=center, text width=.8cm}, 
    xtick={0,...,7},
    xticklabels = {0.5, 0.75, 1, 1.25, 1.5, 2,  2.5, 2.75},
    xlabel={QPS},
    % xmode=log,
    y label style={align=center, text width=3cm}, % Setting alignment is needed to add a line break in axis label
    ylabel={Carbon Emission\\(gCO\textsubscript{2}/token)},
    % tickwidth= 5pt,
    xtick style={draw=none},
    ymajorgrids=true,
    % grid style=dashed,
    legend columns=1,
    legend cell align=left,
    legend style={
        cells={align=left},
        anchor=north,
        at={(0.8,0.97)},
        draw=none,
        fill=none,
        column sep=1ex,
    },
    legend image code/.code={%
        \draw[#1,draw=none] (0cm,-0.07cm) rectangle (0.17cm,0.12cm);
    }
}
]

\begin{axis}[bar shift=6pt]
\addplot+[draw=none,fill=kaito,opacity=0.25] table[col sep=comma, y=v100_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_300m.csv};
\addplot+[draw=none,fill=orange] table[col sep=comma, y=v100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_300m.csv};\label{dsd_300m_300m_v100}

\end{axis}



\begin{axis}[hide axis, bar shift=0pt]
\addplot+[
    draw=none,
    fill=kaito,opacity=0.25] table[col sep=comma, y=t4_a100_carbon_pertoken,  x expr=\coordindex]{fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_300m.csv};\label{dsd_300m_300m_a100_dist};
\addplot+[draw=none,fill=green!70!black] table[col sep=comma, y=t4_carbon_pertoken,   x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_300m.csv};\label{dsd_300m_300m_plot_t4}

\end{axis}


\begin{axis}[hide axis, bar shift=-6pt]

\addplot+[draw=none,fill=blue] table[col sep=comma, y=a100_std,  x expr=\coordindex] {fig/csv/dsd_carbon_emission_data/longbench_carbon_per_token_300m.csv};

\addlegendentry{A100 only}
\addlegendimage{/pgfplots/refstyle=dsd_300m_300m_plot_t4}\addlegendentry{T4}
\addlegendimage{/pgfplots/refstyle=dsd_300m_300m_v100}\addlegendentry{V100}
\addlegendimage{/pgfplots/refstyle=dsd_300m_300m_a100_dist}\addlegendentry{A100 Dist}


\end{axis}



\end{tikzpicture}

==> fig/tikz/dsd_carbon_saving/humaneval.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=2 by 1, % 2 subplots in one row
            horizontal sep=1cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.5\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
    ylabel={Carbon Emission Savings (\%)}, % Lengthy label for the left plot
    ymin=-30, ymax=15, % Specific range for the left subplot
    ytick = {-30,-20,-10,0,10,20},
    yticklabels={-30,-20,-10,0,10,20},
    legend to name=dsd_cs_he_sharedlegend, % Shared legend reference
    legend columns=2,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/humaneval_carbon_savings_300m.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/humaneval_carbon_savings_300m.csv};
\legend{T4 Carbon Saving, V100 Carbon Saving};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=-25, ymax=30, % Different range for the right subplot
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/humaneval_carbon_savings_1b.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/humaneval_carbon_savings_1b.csv};

\end{groupplot}
% \node at ($(group c1r1.north)+(1.8cm,0.4cm)$) {\ref{dsd_cs_he_sharedlegend}};
    \node at ($(group c1r1.north)+(1.8cm,0.4cm)$) {\pgfplotslegendfromname{dsd_cs_he_sharedlegend}};

\node[below=0.8cm of group c1r1.south, anchor=north] {300M};
\node[below=0.8cm of group c2r1.south, anchor=north] {1B};
\end{tikzpicture}


==> fig/tikz/dsd_carbon_saving/longbench.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=2 by 1, % 2 subplots in one row
            horizontal sep=1cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.5\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
    ylabel={Carbon Emission Savings (\%)}, % Lengthy label for the left plot
    ymin=-30, ymax=7, % Specific range for the left subplot\
    ytick = {-30,-20,-10,  0,10},
    yticklabels={-30,-20,-10,  0,10},
    legend to name=dsd_cs_lb_sharedlegend, % Shared legend reference
    legend columns=2,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/longbench_carbon_savings_300m.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/longbench_carbon_savings_300m.csv};
\legend{T4 Carbon Saving, V100 Carbon Saving};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=-40, ymax=12, % Different range for the right subplot
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/longbench_carbon_savings_1b.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/longbench_carbon_savings_1b.csv};

\end{groupplot}
% \node at ($(group c1r1.north)+(1.8cm,0.4cm)$) {\ref{dsd_cs_lb_sharedlegend}};
\node at ($(group c1r1.north)+(1.8cm,0.4cm)$) {\pgfplotslegendfromname{dsd_cs_lb_sharedlegend}};
\node[below=0.8cm of group c1r1.south, anchor=north] {300M};
\node[below=0.8cm of group c2r1.south, anchor=north] {1B};
\end{tikzpicture}


==> fig/tikz/dsd_carbon_saving/sharegpt_1b.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=3 by 1, % 2 subplots in one row
            horizontal sep=0.65cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.42\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
    ylabel={Carbon Emission Savings (\%)}, % Lengthy label for the left plot
    ymin=-30, ymax=30, % Specific range for the left subplot
    ytick = {-30,-15,0,15,30},
    yticklabels={-30,-15,0,15,30},
    legend to name=dsd_cs_sg_1b_sharedlegend, % Shared legend reference
    legend columns=2,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_25p_carbon_savings_1b.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_25p_carbon_savings_1b.csv};
\legend{T4 Carbon Saving, V100 Carbon Saving};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=-40, ymax=25, % Different range for the right subplot
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_median_carbon_savings_1b.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_median_carbon_savings_1b.csv};
% \legend{T4 Carbon Saving, V100 Carbon Saving};
% add additional line


\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=-40, ymax=25, % Different range for the right subplot
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_75p_carbon_savings_1b.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_75p_carbon_savings_1b.csv};


\end{groupplot}
\node at ($(group c2r1.north)+(0,0.4cm)$) {\pgfplotslegendfromname{dsd_cs_sg_1b_sharedlegend}};
\node[below=0.8cm of group c1r1.south, anchor=north] {\small (24,24)};
\node[below=0.8cm of group c2r1.south, anchor=north] {\small (160,140)};
\node[below=0.8cm of group c3r1.south, anchor=north] {\small (510,357)};
\end{tikzpicture}


==> fig/tikz/dsd_carbon_saving/sharegpt_300m.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=3 by 1, % 2 subplots in one row
            horizontal sep=0.65cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.42\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
    ylabel={Carbon Emission Savings (\%)}, % Lengthy label for the left plot
    ymin=-30, ymax=30, % Specific range for the left subplot
    ytick = {-30,-15,0,15,30},
    yticklabels={-30,-15,0,15,30},
    legend to name=dsd_cs_sg_300m_sharedlegend, % Shared legend reference
    legend columns=2,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_25p_carbon_savings_300m.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_25p_carbon_savings_300m.csv};
\legend{T4 Carbon Saving, V100 Carbon Saving};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=-30, ymax=10, % Different range for the right subplot
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_median_carbon_savings_300m.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_median_carbon_savings_300m.csv};
% \legend{T4 Carbon Saving, V100 Carbon Saving};
% add additional line


\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=-40, ymax=15, % Different range for the right subplot
]
\addplot+[
    draw=green!60!black,
    mark options={scale=0.85, fill=green!60!black},
    mark=triangle*,
    line width=0.25mm, 
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=Carbon Saving (A100+T4)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_75p_carbon_savings_300m.csv};
\addplot+[
    draw=orange!90!black,
    mark options={scale=0.8, fill=orange!90!black},
    mark=square*,
    line width=0.25mm,
] table[x=QPS, y=Carbon Saving (A100+V100)
,col sep=comma] {fig/csv/dsd_carbonsaving_data/sharegpt_75p_carbon_savings_300m.csv};


\end{groupplot}
\node at ($(group c2r1.north)+(0,0.4cm)$) {\pgfplotslegendfromname{dsd_cs_sg_300m_sharedlegend}};
\node[below=0.8cm of group c1r1.south, anchor=north] {\small (24,24)};
\node[below=0.8cm of group c2r1.south, anchor=north] {\small (160,140)};
\node[below=0.8cm of group c3r1.south, anchor=north] {\small (510,357)};
\end{tikzpicture}


==> fig/tikz/dsd_slo/slo_humaneval.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=2 by 1, % 2 subplots in one row
            horizontal sep=1cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.5\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
    ylabel={SLO Attainment (\%)}, % Lengthy label for the left plot
    ymin=0, ymax=105, % Specific range for the left subplot
    legend to name=dsd_he_slo_sharedlegend, % Shared legend reference
    legend columns=3,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/humaneval_slo_att_300m.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/humaneval_slo_att_300m.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/humaneval_slo_att_300m.csv};
\legend{A100 only, A100+V100, A100+T4};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=0, ymax=105, % Different range for the right subplot
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/humaneval_slo_att_1b.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/humaneval_slo_att_1b.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/humaneval_slo_att_1b.csv};

\end{groupplot}
% \node at ($(group c1r1.north)+(1.8cm,0.4cm)$) {\ref{sharedlegend}};
\node at ($(group c1r1.north)+(1.8cm,0.4cm)$) {\pgfplotslegendfromname{dsd_he_slo_sharedlegend}};
\node[below=0.8cm of group c1r1.south, anchor=north] {300M};
\node[below=0.8cm of group c2r1.south, anchor=north] {1B};
\end{tikzpicture}


==> fig/tikz/dsd_slo/slo_longbench.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=2 by 1, % 2 subplots in one row
            horizontal sep=1cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.5\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
    ylabel={SLO Attainment (\%)}, % Lengthy label for the left plot
    ymin=0, ymax=105, % Specific range for the left subplot
    legend to name=dsd_lb_slo_sharedlegend, % Shared legend reference
    legend columns=3,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/longbench_slo_att_300m.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/longbench_slo_att_300m.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/longbench_slo_att_300m.csv};
\legend{A100 only, A100+V100, A100+T4};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=0, ymax=105, % Different range for the right subplot
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/longbench_slo_att_1b.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/longbench_slo_att_1b.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/longbench_slo_att_1b.csv};

\end{groupplot}
\node at ($(group c1r1.north)+(1.8cm,0.4cm)$) {\pgfplotslegendfromname{dsd_lb_slo_sharedlegend}};
\node[below=0.8cm of group c1r1.south, anchor=north] {300M};
\node[below=0.8cm of group c2r1.south, anchor=north] {1B};
\end{tikzpicture}


==> fig/tikz/dsd_slo/slo_sharegpt_1b.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=3 by 1, % 2 subplots in one row
            horizontal sep=0.65cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.42\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
   ylabel={SLO Attainment (\%)}, % Lengthy label for the left plot
    ymin=0, ymax=105, % Specific range for the left subplot
    legend to name=dsd_sg_1b_slo_sharedlegend, % Shared legend reference
    legend columns=3,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_25p_slo_att_1b.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_25p_slo_att_1b.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_25p_slo_att_1b.csv};
\legend{A100 only, A100+V100, A100+T4};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=0, ymax=105, % Different range for the right subplot
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_median_slo_att_1b.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_median_slo_att_1b.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_median_slo_att_1b.csv};
% \legend{T4 Carbon Saving, V100 Carbon Saving};
% add additional line


\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=0, ymax=105, % Different range for the right subplot
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_75p_slo_att_1b.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_75p_slo_att_1b.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_75p_slo_att_1b.csv};


\end{groupplot}
% \node at ($(group c2r1.north)+(0,0.4cm)$) {\ref{sharedlegend}};
\node at ($(group c2r1.north)+(0,0.4cm)$) {\pgfplotslegendfromname{dsd_sg_1b_slo_sharedlegend}};
\node[below=0.8cm of group c1r1.south, anchor=north] {\small (24,24)};
\node[below=0.8cm of group c2r1.south, anchor=north] {\small (160,140)};
\node[below=0.8cm of group c3r1.south, anchor=north] {\small (510,357)};
\end{tikzpicture}


==> fig/tikz/dsd_slo/slo_sharegpt_300m.tex <==
\begin{tikzpicture}

\begin{groupplot}[
        group style={
            group size=3 by 1, % 2 subplots in one row
            horizontal sep=0.65cm, % Separation between plots
            vertical sep=0cm % Not used here since only one row
        },
        width=0.42\linewidth, % Width of each subplot
        height=4cm, % Height of each subplot,
        tick label style={font=\footnotesize}, % Decrease tick label font size
        label style={font=\footnotesize}, % Decrease axis label font size
        ymajorgrids=true,
        xtick style={draw=none},ytick style={draw=none}
    ]
    
% First subplot (Left)
\nextgroupplot[
    xlabel={QPS},
    label style={font=\footnotesize},
   ylabel={SLO Attainment (\%)}, % Lengthy label for the left plot
    ymin=0, ymax=105, % Specific range for the left subplot
    legend to name=dsd_sg_300m_slo_sharedlegend, % Shared legend reference
    legend columns=3,
    legend cell align=left,
    legend style={draw=none,fill=none,anchor=north,at={(0.5,1.22)}, text=black,font=\small,      
    column sep=1ex},
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_25p_slo_att_300m.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_25p_slo_att_300m.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_25p_slo_att_300m.csv};
\legend{A100 only, A100+V100, A100+T4};

% \end{axis}
\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=0, ymax=105, % Different range for the right subplot
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_median_slo_att_300m.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_median_slo_att_300m.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_median_slo_att_300m.csv};
% \legend{T4 Carbon Saving, V100 Carbon Saving};
% add additional line


\nextgroupplot[
        xlabel={QPS},
        label style={font=\footnotesize},
        ymin=0, ymax=105, % Different range for the right subplot
]
% A100 only - blue solid line with circles
\addplot+[
     blue,
    solid,
    mark=*,
    mark options={scale=0.8},
    line width=1pt
][% domain=0:1 defines the x-range
domain=0:1] table[x=QPS, y=a100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_75p_slo_att_300m.csv};
% A100+V100 - red dotted line with squares
\addplot+[
    red,
    dotted,
    mark=square*,
    mark options={scale=0.85, fill=red},
    line width=1pt
] table[x=QPS, y=a100_v100_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_75p_slo_att_300m.csv};
% A100+T4 - green dashed line with triangles
\addplot+[
    green!60!black,
    dashed,
    mark=diamond*,
    mark options={scale=1.1, fill=green!60!black},
    line width=1pt
] table[x=QPS, y=a100_t4_slo_attainment
,col sep=comma] {fig/csv/dsd_slo_data/sharegpt_75p_slo_att_300m.csv};


\end{groupplot}
% \node at ($(group c2r1.north)+(0,0.4cm)$) {\ref{sharedlegend}};
\node at ($(group c2r1.north)+(0,0.4cm)$) {\pgfplotslegendfromname{dsd_sg_300m_slo_sharedlegend}};
\node[below=0.8cm of group c1r1.south, anchor=north] {\small (24,24)};
\node[below=0.8cm of group c2r1.south, anchor=north] {\small (160,140)};
\node[below=0.8cm of group c3r1.south, anchor=north] {\small (510,357)};
\end{tikzpicture}


==> tex/z-motivation.tex <==
\section{Motivation}\label{sec:motivation}

To harness disaggregation for carbon reduction, we need to understand the performance, energy consumption, and carbon emissions of different execution components of LLM serving. Thus, we conduct a comprehensive characterization to analyze these metrics across various GPUs and LLM model sizes, as well as the communication overhead. 

We test on three GPU types: A100, V100, and T4. we use randomized text inputs that match the input and output token lengths, as LLM output qualify does not influence the problem we are investigating, 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.99\linewidth]{fig/M_dpd_all.pdf}
	\caption{\textbf{Latency, energy and carbon per token for prefill and decoding phases at different request rates on different GPUs.} The latency SLOs for prefill and decoding are 200ms and 80ms, respectively. Carbon emissions are calculated using the carbon intensity of 261 gCO$_{2}$/kWh from the CISO grid.}\label{fig:m-dpd-all}
\end{figure}


\subsection{Tradeoff Analysis of Prefill and Decoding}\label{subsec:prefill-decode}

We first characterize latency, energy consumption, and carbon emissions on different GPUs for the prefill and decoding phases, separately. We run the Llama-7B model with input and output token lengths of 160 and 140, respectively. 

\paragraph{Latency.} The first row of \Cref{fig:m-dpd-all} shows the latency of the prefill (TTFT) and decoding (TPOT) phases across different GPUs as a function of request rate (number of requests per second). The results reveal two observations. First, TTFT consistently takes longer than TPOT under the same request rate and GPU. This is because the prefill phase, which processes all input tokens in parallel, is more compute intensive than the decoding phase, which outputs tokens sequentially in an autoregressive manner. Second, latency improves with newer GPUs (A100) compared to older GPUs (V100 and T4), which aligns with expectations given the higher compute capability of newer GPUs (as indicated by TFLOPs in \Cref{tbl:spec}).

\paragraph{Energy.} The second row of  \Cref{fig:m-dpd-all} shows the energy consumption per token for the prefill and decoding phases across different GPUs as a function of request rate. The results highlight two findings. First, the decoding phase consumes more energy than the prefill phase under the same request rate and GPU. This is mainly because the total decoding time is much longer than the prefill time. Second, during the prefill phase, older GPUs (V100 and T4) consume more energy than newer GPUs (A100). However, this trend does not hold for decoding. This is because the prefill phase is highly compute-intensive, and newer GPU with greater compute capability can process requests faster and more energy-efficiently compared to older GPU with lower compute capabilities. In contrast, the decoding phase is less compute-intensive, allowing relatively older GPUs to handle requests at lower request rates, thus making them more energy-efficient than newer GPUs.

\paragraph{Carbon.} The last row of \Cref{fig:m-dpd-all} shows the total carbon emissions for the prefill and decoding phases across various GPUs as a function of request rate. The results highlight two findings. First, the prefill phase always produces lower carbon emissions than the decoding phase under the same request rate and GPU. This difference arises because the prefill phase is more compute-intensive than the decoding phase. Second, for the prefill phase, newer GPUs generally exhibit lower carbon emissions compared to older GPUs at the same request rate. However, this trend does not hold for the decoding phase, where T4 can have lower carbon emissions than A100. 

\paragraph{\underline{Takeaway \#1.}} The prefill and decoding phases exhibit different behaviors in terms of latency, energy, and carbon. While decoding is more energy-intensive, older GPUs can be more energy- and carbon-efficient for decoding compared to prefill as decoding is less compute-intensive. By strategically assigning each phase to appropriate GPU types, we can reduce total carbon emissions without compromising performance. Unlike prior work like DistServe~\cite{zhong2024distserve} and Splitwise~\cite{patel2024splitwise} that focused on disaggregating prefill and decoding phases for performance and cost optimization, this paper prioritizes minimizing total carbon emissions.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{fig/model_sizes_latency_vs_QPS.pdf}
	\caption{\textbf{TTFT (prefill) and TPOT (decoding) of different model sizes at different request rates on different GPUs.} The latency SLOs for prefill (TTF) and decoding (TPOT) phases are 200ms and 80ms, respectively. }\label{fig:m-latency-size}
\end{figure}

\subsection{Analysis of LLM Model Size}\label{subsec:model-size}

We characterize latency and energy consumption for various Llama model sizes (300M, 1B, and 7B) with input and output token lengths of 160 and 140.

\paragraph{Latency.} \Cref{fig:m-latency-size} shows the latency of the prefill (TTFT) and decoding (TPOT) of different model sizes at different request rates across different GPU types as a function of request rate. The latency SLOs for TTFT and TPOT are 1000ms and 80ms, respectively. The results highlight three key findings. First, as model size increases, both TTPT and TPOT increase across all GPU types due to greater compute demands, leading to longer processing times. Second, larger model sizes reduce the request rate that can meet latency SLOs, with the largest models (7B) potentially failing to meet SLOs at any request rate. Third, at many request rates, older GPUs (V100, T4) can meet latency SLOs comparable to newer GPUs (A100), particularly for smaller models, revealing opportunities for using older GPU effectively.  

\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{fig/model_sizes_energy_per_token_vs_QPS.pdf}
	\caption{\textbf{Energy per token of different model sizes at different request rates on different GPUs.}  }\label{fig:m-energy-size}
\end{figure}

\paragraph{Energy.} \Cref{fig:m-energy-size} shows the energy consumption per token of different model sizes on different GPUs as a function of the request rate. The results highlight three key findings. First, energy increases with model size across all GPU types at the same request rate due to higher processing times and greater compute demands.  
Second, as request size grows, energy per token generally decreases. This is because larger requests improve GPU utilization, allowing the GPU to operate closer to its thermal design power (TDP). At this point, token throughput increases faster than power usage, stabilizing energy consumption per token when the GPU reaches optimal throughput within its TDP.  
Third, older GPUs (V100, T4) tend to be more energy-efficient than newer GPUs (A100) for smaller models (300M, 1B). However, this advantage diminishes for larger models like 7B, where older GPUs are only more energy-efficient at low request rates.  

\paragraph{\underline{Takeaway \#2.}} Small size models can meet comparable latency SLOs as larger models at certain request rates, even on older GPUs, while providing significantly better energy efficiency. For less complex LLM tasks, replacing large models on newer GPUs with smaller ones on older GPUs could be more energy- and carbon-efficient.

\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=\linewidth]{fig/M_bandwidth_need}  \vspace{-0.1in}
	\end{center}\vspace{-0.3in}
	\caption{\textbf{Bandwidth requirement comparisons between \DistPD{} (DPD) and \DistSD (DSD) when connecting A100 and T4/V100.} DPD experiments the 7B model, with prefill on A100 and decoding on T4/V100. For DSD, the 7B target model runs on A100, while the 1B or 300M draft model runs on T4/V100.}\label{fig:bandwidth}
\end{figure}


\subsection{Analysis of Bandwidth Requirement}\label{subsec:bandwidth}

As discussed in~\cref{subsec:related}, a key limitation of disaggregating the prefill and decoding phases is the high bandwidth requirement due to the large KV cache size. Although prior work like DistServe~\cite{zhong2024distserve} and SplitWise~\cite{patel2024splitwise} discusses this issue, their solutions depend on high-end homogeneous or heterogeneous GPUs equipped with advanced networking devices such as NVLink. However, this limitation persists in scenarios where high network connectivity is unavailable and becomes even more pronounced when data transfers occur between heterogeneous GPUs---where one is high-end and the other is older and lower-tier. In such cases, performance gains diminish and carbon reduction benefits are also reduced.  

\Cref{fig:bandwidth} illustrates the bandwidth limitations when connecting heterogeneous GPUs, such as A100 and T4/V100, with a 16Gbps bandwidth cap. The results show that when serving the LLaMA 7B model and transferring the KV cache between an A100 and T4/A100, the system quickly encounters out-of-memory (OOM) issues as QPS increases.  

To overcome this challenge, we identify a second use case based on speculative decoding. In the experiments, the target model is 7B, while the draft models are smaller (1B and 300M). As shown in \Cref{fig:bandwidth}, \DistSD{} requires 10$\times$ \todo{double check the number} less bandwidth than \DistPD{} over a wide range of QPS since it only transfers tokens rather than the large KV cache.  

\paragraph{\underline{Takeaway \#3.}} \DistPD{} is feasible only when high network connectivity is available. Otherwise, \DistSD{} is an alternative for reducing carbon emissions.



% \begin{figure}[t]
% 	\centering
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/M_disagg_Prefill-Energy}
% 		\caption{Prefill energy.}
% 		\label{fig:m-energy-prefill}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/M_disagg_Decoding-Energy}
% 		\caption{Decoding energy.}
% 		\label{fig:m-energy-decoding}
% 	\end{subfigure}
% 	\caption{Energy per token for the prefill and decoding phases at different request rates across different GPUs. }\label{fig:m-energy}
% \end{figure}

% \begin{figure}[t]
% 	\centering
%	\begin{subfigure}[b]{0.49\linewidth}
%		\includegraphics[width=1\linewidth]{fig/M_disagg_Prefill-Operational-Carbon}
%		\caption{Prefill operational carbon.}
%		\label{fig:m-op-prefill}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.49\linewidth}
%		\includegraphics[width=1\linewidth]{fig/M_disagg_Decoding-Operational-Carbon}
%		\caption{Decoding operational carbon.}
%		\label{fig:m-op-decoding}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.49\linewidth}
%		\includegraphics[width=1\linewidth]{fig/M_disagg_Prefill-Embodied-Carbon}
%		\caption{Prefill embodied carbon.}
%		\label{fig:m-em-prefill}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.49\linewidth}
%		\includegraphics[width=1\linewidth]{fig/M_disagg_Decoding-Embodied-Carbon}
%		\caption{Decoding embodied carbon.}
%		\label{fig:m-em-decoding}
%	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/M_disagg_Prefill-Total-Carbon}
% 		\caption{Prefill total carbon.}
% 		\label{fig:m-total-prefill}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/M_disagg_Decoding-Total-Carbon}
% 		\caption{Decoding total carbon.}
% 		\label{fig:m-total-decoding}
% 	\end{subfigure}
% 	\caption{Total carbon emissions per token for the prefill and decoding phases at different request rates across different GPUs. The analysis uses the carbon intensity value of 261 gCO$_{2}$ from the CISO grid.}\label{fig:m-carbon}
% \end{figure}


% \begin{figure}[t]
% 	\centering
% 	\begin{subfigure}[b]{0.33\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/energy_per_token_vs_QPS_300m}
% 		\caption{Energy 300M.}
% 		\label{fig:m-e-300m}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.325\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/energy_per_token_vs_QPS_1b}
% 		\caption{Energy 1B.}
% 		\label{fig:m-e-1b}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.325\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/energy_per_token_vs_QPS_7b}
% 		\caption{Energy 7B.}
% 		\label{fig:m-e-7b}
% 	\end{subfigure}
% 	\caption{Energy per token of different model sizes at different request rates across different GPUs.}\label{fig:m-energy-size}
% \end{figure}


% \begin{figure}[t]
% 	\centering
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/TTFT_vs_QPS_300m}
% 		\caption{TTFT Llama-300M.}
% 		\label{fig:m-ttft-300m}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/TPOT_vs_QPS_300m}
% 		\caption{TPOT Llama-300M.}
% 		\label{fig:m-tpot-300m}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/TTFT_vs_QPS_1b}
% 		\caption{TTFT Llama-1B.}
% 		\label{fig:m-ttft-1b}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/TPOT_vs_QPS_1b}
% 		\caption{TPOT Llama-1B.}
% 		\label{fig:m-tpot-1b}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/TTFT_vs_QPS_7b}
% 		\caption{TTFT Llama-7B.}
% 		\label{fig:m-ttft-7b}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\linewidth}
% 		\includegraphics[width=1\linewidth]{fig/TPOT_vs_QPS_7b}
% 		\caption{TPOT Llama-7B.}
% 		\label{fig:m-tpot-7b}
% 	\end{subfigure}
% 	\caption{\textbf{TTFT (prefill) and TPOT (decoding) of different model sizes at different request rates on different GPUs.}}\label{fig:m-latency-size}
% \end{figure}
